Self-Managing DRAM: A Low-Cost Framework for Enabling Autonomous and Efficient in-DRAM Operations

The memory controller is in charge of managing DRAM maintenance operations (e.g., refresh, RowHammer protection, memory scrubbing) to reliably operate modern DRAM chips. Implementing new maintenance operations often necessitates modifications in the DRAM interface, memory controller, and potentially other system components. Such modifications are only possible with a new DRAM standard, which takes a long time to develop, likely leading to slow progress in the adoption of new architectural techniques in DRAM chips. We propose a new low-cost DRAM architecture, Self-Managing DRAM (SMD), that enables autonomous in-DRAM maintenance operations by transferring the responsibility for controlling maintenance operations from the memory controller to the SMD chip. To enable autonomous maintenance operations, we make a single modification to the DRAM interface, such that an SMD chip rejects memory controller accesses to DRAM regions under maintenance, while allowing memory accesses to others. Thus, SMD enables 1) implementing new in-DRAM maintenance mechanisms (or modifying existing ones) with no further changes in the DRAM interface or other system components, and 2) overlapping the latency of a maintenance operation in one DRAM region with the latency of accessing data in another. We evaluate SMD and show that it 1) can be implemented without adding new pins to the DDRx interface with low latency and area overhead, 2) achieves 4.1% average speedup across 20 four-core memory-intensive workloads over a DDR4-based system/DRAM co-design technique that intelligently parallelizes maintenance operations with memory accesses, and 3) guarantees forward progress for rejected memory accesses. We believe and hope SMD can enable innovations in DRAM architecture to rapidly come to fruition. We open source all SMD source code and data at https://github.com/CMU-SAFARI/SelfManagingDRAM.

==> sections/_1_revision_summary.tex <==
\thispagestyle{empty} % No page number
\onecolumn
\setstretch{0.90}
\noindent We thank the reviewers for their valuable feedback. We {addressed reviewer concerns and improved the paper's clarity in this revision, as summarized on this page.} In this document, we use \iqrev{blue for responding to individual questions and concerns}. We will further improve the paper for the next (shepherd or camera-ready) version.

{\noindent\bf{Individual questions}} labeled as: \textbf{IQ[Reviewer ID][Question Number]}, e.g., Reviewer A's first question is IQA1.

\vspace{0.5em}
\hrule
\vspace{0.5em}

\noindent
\textbf{IQA1: Evaluate more optimized ACT\_NACK rejection approaches.} We add \cref{sec:smd_optimized} that describes and estimates the performance of another version of SMD (similar to the reviewer's description) in the revised paper.

\noindent
\textbf{IQA2: Show the fraction of memory requests that were rejected. How does this fraction change when projecting into more frequent maintenance?} We incorporate the fraction of rejected memory requests 1) for the previously evaluated configurations into revised \cref{subsec:multi_core_perf} and 2) for the new evaluated configurations in \cref{sec:smd_optimized} and \cref{sec:smd_scaling}. Figure~\ref{fig:smd_scaling} in the revised paper shows the rejection rate for more frequent DRAM refresh periods of 16, 8, and 4 milliseconds for SMD-FR. 

\noindent
\textbf{IQA3: The performance benefits of SMD are small considering its 3\% pin overhead.} We highlight text in \cref{sec:intro} and \cref{sec:hw_overhead} to emphasize SMD can be implemented \emph{without} increasing the number of pins. Although SMD's main objective is \emph{not} to improve system performance, we demonstrate in~\cref{sec:evaluation} that \emph{an} SMD design that leverages subarray-level parallelism provides speedups almost as high as those of No-Refresh (that does \emph{not} perform any maintenance operations) for 4c-high workloads.  

% (i.e., the headroom for performance improvement, by further alleviating the overheads of maintenance operations, over SMD-Combined is low).

\noindent
\textbf{IQA4: ECC scrubbing maintenance mechanism does not work with server memory.} Revised \cref{subsec:smd_ecc_scrubbing} describes why rank-level ECC scrubbing and in-DRAM ECC scrubbing should be done separately but in a combined way in server modules.

\noindent
\textbf{IQA5: Clarify per-bank and per-subarray refresh granularity.} Revised \cref{subsec:smd_refresh} clarifies the refresh granularity for per-subarray refresh. Per-bank refresh carries out refresh for multiple rows concurrently.

\vspace{0.5em}
\hrule
\vspace{0.5em}

\noindent
We found some of Reviewer B's terse and thus we believe we might not have precisely addressed them. Could the reviewer provide more feedback? Specifically, we are not sure what details about 1) how ACT\_NACK's are handled and how long to wait for a retry in~\cref{subsec:rejecting_acts} and 2) scheduling changes needed in~\cref{subsubsec:mc_modifications} are missing from the submitted paper.
%our description (that already exists in the submitted version) of 
% how ACT\_NACK's are handled and how long to wait for a retry in~\cref{subsec:rejecting_acts}, and scheduling changes needed in~\cref{subsubsec:mc_modifications}.

\noindent
\textbf{IQB1: Add more details on the impact of ACT\_NACK to MC design.} Please see highlighted text across~\cref{subsec:rejecting_acts} and~\cref{subsubsec:mc_modifications} for detailed description on impact of MC design due to ACT\_NACK. Revised \cref{subsubsec:mc_modifications} describes 1) the overhead of tracking lock regions and 2) the impact of SMD on address mapping schemes in the memory controller. 

\noindent
\textbf{IQB2: How do you avoid a worst-case long tail effect?} The worst-case long tail for a memory request is the time it takes a DRAM chip to perform the most time taking maintenance operation. This is already explained in \cref{subsec:forward-progress} in the submitted paper, now highlighted in the revision. Our simulator properly models the worst-case long tail effect. Our simulator will be open sourced.

\vspace{0.5em}
\hrule
\vspace{0.5em}

\noindent
\textbf{IQC1: Is LRT global and are there latencies within the DRAM that are not accounted for?} We evaluate LRT as a per-bank structure. We describe further how LRT is placed in revised~\cref{sec:sm_dram} and~\cref{sec:hw_overhead}.

\noindent
\textbf{IQC2: ALERT pin is slow and imprecise.} We incorporate the reviewer's comment into revised \cref{sec:hw_overhead}.

\vspace{0.5em}
\hrule
\vspace{0.5em}

\noindent
\textbf{IQD1: Co-design overhead is understated.} We highlight text (from the submitted paper) that describes the overheads of \mech{} in the revised paper. These highlights are in~\cref{sec:intro} and~\cref{sec:hw_overhead}. We will describe any missing co-design overheads in the next version of our paper if the reviewer provides more feedback.

\noindent
\textbf{IQD2: In-DRAM scrubbing information should be exposed.} We discuss how \mech{} does \emph{not} preclude exposing in-DRAM scrubbing information in Section~\ref{subsec:smd_ecc_scrubbing} in the revised paper.

\noindent
\textbf{IQD3: The need to speculate on the reason of an ACT\_NACK to decide on the next action would raise the complexity of MC non-trivially.} We evaluate \mech{} using a simple MC that does \emph{not} speculate on the reason of ACT\_NACKs. This design already provides 88.3\% of the speedups provided by No-Refresh (that completely mitigates the overhead of maintenance operations), on average across all evaluated 4c-high workloads. We leave the extensive evaluation of memory controller designs suggested by the reviewer for future work. In fact, we believe \mech{} enables new MC designs that can provide other benefits, but these are out of the scope of our submission.
% There is something here. We should not fully dismiss this comment. Maybe say this happens rarely and the effects are such and such (quantitative).  The new section should emphasize the results we get with a simple MC.

\noindent
\textbf{IQD4: Forward progress is likely not guaranteed.} In an ARI of \SI{62.5}{\nano\second}, the memory controller has enough time to serve multiple READ requests to a DRAM row other than the ACT\_NACK'd row and still issue an activate command to the ACT\_NACK'd row at the end of every ARI. Revised \cref{subsec:forward-progress} incorporates our response.
% We elaborate on our claim that our implementation of \mech{} ensures forward memory progress to explain how this implementation of \mech{} deals with the example raised by the reviewer in revised Section~\ref{sec:XYZ}.

\vspace{0.5em}
\hrule
\vspace{0.5em}

\noindent
\textbf{IQE1: It is not clear what the root cause of the difficulty is in adopting maintenance operations to the DRAM standards.} We incorporate the reviewer's comments into revised~\cref{sec:intro} and~\cref{sec:drawbacks_current_maintenance}.
% Reason 1) DDRx did not evolve too slowly because of maintenance ops 2) not all standards move slowly.

\noindent
\textbf{IQE2: ACT\_NACK divergence implies that you cannot wire ACT\_NACK pins from different chips to the single processor pin.} The submitted paper does \emph{not} introduce ACT\_NACK divergence because we do \emph{not} present variable rate refresh as a use case. The reviewer's comment, which had been addressed in a past revision, is outdated.

\noindent
\textbf{IQE3: It is unclear if SMD reduces the overall complexity of a computing system.} We do not claim to reduce overall complexity as our goal. Our goal is to enable easier adoption of new ideas and progress. That said, complexity may not change that much or may even reduce. We note that ``overall complexity'' is not easy to evaluate. 

\noindent
\textbf{IQE4: Why not use request-reply interfaces? Discuss the design philosophy of SMD in high-level.} SMD is part of a continuum between fully master-slave and fully request-reply interfaces. It tries to achieve a balance that enables faster innovation and easier adoption of new ideas. We incorporate our response into revised \cref{sec:sm_dram}.

\noindent
\textbf{IQE5: Isolate the benefits of SMD from single-bank refresh, SALP, Graphene.} The evaluated ``MC-Combined-DSARP'' configuration (described in~\cref{sec:methodology}) combines single-bank intelligent refresh, SALP, and Graphene in the memory controller. We highlight the benefits SMD provides over ``MC-Combined-DSARP'' in revised~\cref{sec:evaluation}.

\setstretch{0.936}
